Far Away in the Deep Space: Dense Nearest-Neighbor-Based Out-of-Distribution Detection

The key to out-of-distribution detection is density estimation of the in-distribution data or of its feature representations. This is particularly challenging for dense anomaly detection in domains where the in-distribution data has a complex underlying structure. Nearest-Neighbors approaches have been shown to work well in object-centric data domains, such as industrial inspection and image classification. In this paper, we show that nearest-neighbor approaches also yield state-of-the-art results on dense novelty detection in complex driving scenes when working with an appropriate feature representation. In particular, we find that transformer-based architectures produce representations that yield much better similarity metrics for the task. We identify the multi-head structure of these models as one of the reasons, and demonstrate a way to transfer some of the improvements to CNNs. Ultimately, the approach is simple and non-invasive, i.e., it does not affect the primary segmentation performance, refrains from training on examples of anomalies, and achieves state-of-the-art results on RoadAnomaly, StreetHazards, and SegmentMeIfYouCan-Anomaly.

==> tables/fs_laf.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|c|rr}
    \toprule
        Method & OE & \multicolumn{1}{c}{AP} & \multicolumn{1}{c}{FPR$_{95}$}\\
        \midrule
        SML~\cite{Jung_2021_ICCV}     & & 36.55 & 14.53\\
        PEBAL~\cite{Tian2021}   & $\checkmark$ & 59.83 & 6.49 \\ 
        % M2F & & 52.0 & 20.5 \\
        % NLS & & 60.68 & 13.45\\
        % NLS+OE & \checkmark & 69.37 & 10.04 \\
        \midrule
        Segmenter-B (Ours) & & 56.13 & 24.59 \\
        SETR (Ours) & & 56.66 & 24.68 \\
        \midrule
        Segmenter-B (Ours) & $\checkmark$  & 64.75 & 18.06 \\
    \bottomrule
    \end{tabular}
    \caption{Performance on Fishyscapes LostAndFound-val. \todo{}}
    \label{tab:laf}
\end{table}


==> tables/selfsup.tex <==
\begin{table}
\centering
\begin{tabular}{l|ccc}
               & \multicolumn{3}{c}{RoadAnomaly}  \\
               & AUC  & AP   & FPR$_{95}$         \\
\midrule                             
R50 supervised  & 87.3 & 39.4 & 31.5                \\
R50	\ma{rnd?}   & 87.3 & 36.9 & 34.4                \\
R50 DINO        & 85.5 & 36.3 & 37.6                \\
R50 RSB	        & 88.0 & 41.7 & 31.4                \\
\midrule   
ViT supervised  & 94.7 & 70.0 & 15.7                \\
ViT DeiT        & 82.8 & 44.7 & 45.7                \\
ViT iBOT        & 93.3 & 59.0 & 18.5                \\
ViT DINO        & 94.5 & 60.1 & 16.9                \\
\end{tabular}
\caption{Results for self-supervised features or pre-training. NN only, no combination. \ma{not referenced in text yet. add citations. RSB outperforms supervised!}}
\label{tab:selfsup}
\end{table}

==> tables/smiyc_anomaly.tex <==
% this isn't used: see all_single_row

%%%%%%%%%%%%%%%%%%%%%%% OLDER VERSION %%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[h]
%     % \small
%     \centering
%     \begin{tabular}{l|c|rr}
%     \toprule
%     Method      & OE         & AP $\uparrow$    & FPR$_{95}\downarrow$ \\
%     \midrule
%     PEBAL\cite{Tian2021}& \checkmark & 49.1 & 40.8 \\
%     NFlowJS\cite{Grcic2021DenseAD}     &            & 56.9 & 34.7 \\
%     ObsNet\cite{Besnier2021}      &            & 75.4 & 26.7 \\
%     DenseHybrid\cite{Grcic2022} & \checkmark & 78.0 & {9.8} \\
%     Max-Entropy\cite{Chan2021EntropyMA} & \checkmark & {85.5} & 15.0 \\
%     % M2F & & 76.3 & 93.9 \\
%     % NLS & & {86.1} & 15.9\\
%     % NLS+OE & \checkmark & 91.3 & 10.7\\
%     \midrule
%     cDNP-Segmenter-B (Ours)&            & {88.9}  & {11.4} \\
%     \bottomrule
%     \end{tabular}
%     \caption{State of the art results on the SMIYC-Anomaly benchmark (test set, official leaderboard). OE denotes the use of negative/anomalous training data. Best results are bold, second best are underlined. \todo{bold no OE?}} 
%     \label{tab:sota_smiyc}
% \end{table}

==> tables/sota.tex <==
\begin{table}
\centering
\small
\setlength{\tabcolsep}{5pt}
\scriptsize
\begin{tabular}{l|c|cccc}
\toprule
     & & \multicolumn{2}{c}{RoadAnomaly} & \multicolumn{2}{c}{StreetHazards}\\
    Method & OE & AP$\uparrow$ & FPR$_{95}\downarrow$ & AP$\uparrow$ & FPR$_{95}\downarrow$\\
    \midrule
    % SynthCP\cite{Xia2020} & & 24.9 & 64.7 & 9.3 & 28.4\\
    % SML\cite{Jung_2021_ICCV} & & 25.8 & 49.7 & - & - \\
    DML\cite{cen2021deep} & & 37.0 & 37.0 & 14.7 & 17.3 \\
    % Synboost\cite{Biase2021} & \checkmark & 41.8 & 59.7 & - & -\\
    MOoSe\cite{moose} &  & 43.6 & 32.1 & 15.2 & 17.6\\
    PEBAL\cite{Tian2021} & \checkmark & 62.4 & 28.3 & - & - \\
    DenseHybrid\cite{Grcic2022} & \checkmark & - & - & 30.2 & 13.0 \\
    % M2F                         &            & 66.7  & 13.4 & - & - \\
    % NLS                         &            & 78.5 & 12.7 & - & - \\
    % NLS+OE                      & \checkmark & 84.1 & {9.7} & - & - \\
    \midrule
    cDNP-ConvNeXt-S (Ours) & & 69.6 & 19.1 & {31.2} & {12.8} \\
    cDNP-Segmenter-B (Ours) & & {85.6} & {9.8} & {46.2} & 14.9 \\
    cDNP-SETR (Ours) &   & {85.9} & {13.8} & - & - \\
    \bottomrule
\end{tabular}
\caption{cDNP obtains state of the art results for both RoadAnomaly and StreetHazards, AP and FPR$_{95}$. OE denotes the use of negative/anomalous training data, according to each specific approach. Best results are bold, second best are underlined.}
\label{tab:sota_ra_sh}
\end{table}

